On inverse shadowing

We give a reformulation of the inverse shadowing property with respect to the class of all pseudo-orbits. This reformulation bears witness to the fact that the property is far stronger than might initially seem. We give some implications of this reformulation, in particular showing that systems with inverse shadowing are not sensitive. Finally we show that, on compact spaces, inverse shadowing is equivalent to a finite version of it.

==> Sections/Introduction.tex <==
Let $f\colon X\to X$ be a continuous function on a metric space $X$. A $\delta$\textit{-pseudo-orbit} is a sequence $(x_i)_{i\in \omega}$ such that $d(f(x_{i}),x_{i+1}) <\delta$ for all $i\in\omega$. Pseudo-orbits are of importance when calculating an orbit numerically, as rounding errors mean a computed orbit will be a pseudo-orbit. The sequence $(y_i)$ from $X$ is said to $\epsilon$-shadow the sequence $(x_i)$ provided $d(y_i,x_i)<\epsilon$ for all $i$. Loosely, a system is said to have \textit{shadowing}, or \textit{the pseudo-orbit tracing property}, if pseudo-orbits are shadowed by true orbits. %Thus, if a system has shadowing then computed orbits are followed by true trajectories. 
Shadowing is important when modelling a system numerically (for example \cite{Corless, Pearson}). However, it is also important theoretically. For example, Bowen \cite{bowen-markov-partitions} used shadowing implicitly as a key step in his proof that the nonwandering set of an Axiom A diffeomorphism is a factor of a shift of finite type. Since then it has been studied extensively, in the setting of numerical analysis \cite{Corless,CorlessPilyugin,Pearson}, as a key factor in stability theory \cite{Pilyugin, robinson-stability,WaltersP}, in understanding the structure of $\omega$-limit sets and Julia sets, 
\cite{
barwell-davies-good,
BarwellGoodOprochaRaines, 
BarwellMeddaughRaines2015, 
BarwellRaines2015,
Bowen, 
MeddaughRaines}, and as a property in and of itself \cite{Coven, fernandez-good, GoodMeddaugh2018, LeeSakai, Nusse, Pennings, Pilyugin,Sakai2003}.
 
 
 First introduced by Corless and Pilyugin \cite{CorlessPilyugin} as something akin to the ``dual'' of shadowing, and as part of the concept of bishadowing by Diamond \textit{et al} \cite{DiamondKozyakinKloedenPokrovskii}, inverse shadowing in a system informally means that true trajectories may be recovered from computed orbits (within some given accuracy).  %Conversely, one may wonder under what circumstances it might be possible to recover true trajectories from computed orbits: it is this line of thinking which leads to \textit{inverse shadowing}.
%Inverse shadowing was first introduced by Corless and Pilyugin \cite{CorlessPilyugin} and as part of the concept of bishadowing by Diamond \textit{et al} \cite{DiamondKozyakinKloedenPokrovskii}. 
Kloeden, Ombach and Pokroskii \cite{KloedenOmbackPokrovskii} later defined inverse shadowing using the notion of a $\delta$-method (defined below). %see \cite{ChoiSungsookLee,DiamondLeeYinghao,Lee, Pilyugin2002} for more on this concept).
Inverse shadowing has since been studied in a variety of settings with respect to various classes of admissible pseudo-orbits \cite{GoodMitchellThomas,Honary, KloedenOmbackPokrovskii,Lee, LeePark, Pilyugin2002}. Of particular interest has been its relationship to structural stability. In \cite{Pilyugin2002} Pilyugin showed that if an Axiom A diffeomorphism on a closed $C^\infty$ manifold is structurally stable, then it has the inverse shadowing property with respect to classes of continuous methods. Meanwhile in \cite{KloedenOmbach} Kloeden and Ombach prove that a structurally stable homeomorphism on a compact space has inverse shadowing with respect to the class of methods induced by homeomorphism. See \cite{ChoiLeeZhang,Honary,Lee}
for more on stability and inverse shadowing. %Whilst clearly of theoretical importance, inverse shadowing has also been studied as a property in and of itself \cite{GoodMitchellThomas}. %Lee and Park \cite{LeePark} show that inverse shadowing with respect to various classes are equivalent to the classical shadowing property for homeomorphisms of the circle. In \cite{GoodMitchellThomas} we show that inverse shadowing is preserved under many induced dynamical systems including inverse limits, symmetric and Tychonoff products and the induced hyperspace of compact sets.  

\medskip

In this paper we examine inverse shadowing, with particular attention to inverse shadowing with respect to the class of all pseudo-orbits. In Section \ref{SectionReform} we prove that inverse shadowing is equivalent to a property which essentially involves a quantifier swap in the definition. We use this reformulation to give a number of implications in Section \ref{SectionImplications}, in particular showing that a system exhibiting inverse shadowing is not \textit{eventually sensitive} (defined below). We conclude by showing that when the phase space is compact, for the classes $\mathcal{T}_0$, $\mathcal{T}_c$ and $\mathcal{T}_h$, inverse shadowing is equivalent to a finite version.

Throughout $(X,d)$ is a metric space: we emphasise that, unless otherwise stated, we do not assume $X$ to be compact. 
We denote by $\mathbb{Z}$ the set of all integers; the set of positive integers $1,2,3,4,\ldots$ is denoted by $\mathbb{N}$ whilst $\omega \coloneqq\mathbb{N}\cup\{0\}$.
